Can Authoritative Governments Abuse the Right to Access?

The right to access is a great tool provided by the GDPR to empower data subjects with their data. However, it needs to be implemented properly otherwise it could turn subject access requests against the subjects privacy. Indeed, recent works have shown that it is possible to abuse the right to access using impersonation attacks. We propose to extend those impersonation attacks by considering that the adversary has an access to governmental resources. In this case, the adversary can forge official documents or exploit copy of them. Our attack affects more people than one may expect. To defeat the attacks from this kind of adversary, several solutions are available like multi-factors or proof of aliveness. Our attacks highlight the need for strong procedures to authenticate subject access requests.

==> 02-basics.tex <==
\section{Right to access}\label{sec:basics}

The right to access one's personal data (Article 15 of GDPR~\cite{EU-679-2016}) via Subject Access Requests (SAR) is fundamental to ensure data protection. It makes the processing of personal data by organizations transparent and accountable towards data subjects, whereby these are made aware of, and can verify the lawfulness of the processing of their data (Recital 63 of GDPR~\cite{EU-679-2016}).

This right to access by individuals complements the mandate of the data protection authorities to monitor and enforce the application of the GDPR (Article 57.1.a of GDPR~\cite{EU-679-2016}). The right to access also enables the exercise of all the other rights (erasure, rectification, restriction, etc). This section presents the background knowledge concerning the scope, exercise and requirements needed to implement the right to access.


\subsection{Scope of the GDPR}

The GDPR (in Article 3) applies to the processing of personal data performed by: (i) data controllers who process personal data in the context of the activities of an organisation in the EU, regardless of whether the processing takes place in the EU or not, and regardless of the nationality of the data subjects (first extraterritoriality effect of the GDPR), (ii) data controllers outside the EU, when they collect personal data from EU residents (second extraterritoriality effect of the GDPR, also known as "\emph{Brussels effect}"~\cite{Anstis2021}). 
 
\subsection{Exercising SAR}

 % More precision on its application are given in Recitals 57, 59, 63 and 64.  
%
%The UK's data protection authority (ICO)~\cite{ICO2017} and the European Data Protection Supervisor (EDPS)~\cite{EDPS2014} have also issued guidelines for the right to access (before the Brexit).
%
% and it is also the only practical right regarding personal data in the Charter of Fundamental Rights of the European Union. 
%
%The cases of Max Schrems vs Facebook~\cite{Schrems2015,Schrems2020} is certainly the best illustration of the power of this right. Schrems sent an access request to Facebook and received a huge PDF file (including data should have been erased).


Both the data controller and processor have an explicit \emph{obligation to facilitate the exercise of data subjects' rights} (Articles 12.1 and 28.3.e). 

\textbf{Modalities of SAR} need to be provided to facilitate the exercise of this right (Recital 59), \emph{e.g.} electronic means to request access, charges, mechanisms of request, and timing. Upon reception of a request, the data controller must take action on the user request within a month, as defined in Article 12.3 of the GDPR.

\textbf{Modes of SAR.}  SAR can be  performed in two modes: \emph{direct} request, whereby a data subject directly requests their data to the data controller; or \emph{indirect} requests (proxy-based SAR), when data subjects need to first submit their requests to a third party. This proxy can be a dedicated organization that manages SAR on behalf of users, a company, a Data Protection Authority (DPA). Indirect requests concerns very specific data controllers (like police or other authorities) and it is not common to submit requests to these authorities. In this paper, we only consider direct requests, but our work can also apply to indirect requests.


\subsection{Authenticating a SAR}

When a data controller receives an access request, it needs to verify that this request is legitimate, in order to avoid data breaches where data of one subject would be sent to a different subject (Article 4.12 of GDPR). If authentication is not enforced, the data of a subject can be collected by anyone impersonating the subject to the data controller.

This authentication has two purposes: i) establish the subject's identity, and ii) verify that the subject's identity matches the requested data, i.e. whether SARs are eligible. Interestingly, in~\cite{Bufalieri2020}, 334 subject access requests were submitted to different data controllers, and 58 organizations provided data without any verification of the subject identity. This demonstrates that the right to access can be easily abused if it is not implemented properly. 

%
%\textbf{Procedural rules for SAR eligibility:}
%\begin{enumerate}
%\item Reasonable measures to verify the identity of the subject. Data controllers should use all reasonable measures to verify the identity of a data subject who requests access, in particular in the context of online services and online identifiers (Recital 64 GDPR).
%\item Not in a position to identify the requester. When the controller is able to demonstrate that it is not in a position to identify the data subject, the controller can deny the request, and shall inform the data subject accordingly (Article 11.2 of GDPR).
%\item Request for additional information whenever there are doubts. 
%Where the controller has reasonable doubts concerning the identity of the subject, the controller may request the provision of additional information necessary to confirm the identity of the data subject  (Article 12.6 of GDPR).
%\item Not obliged to obtain more information to identify users.
%A data controller should not be obliged to acquire additional information in order to identify the data subject for the sole purpose of complying with any provision of this Regulation (Recital 57 of the GDPR). \kao{unclear to me: above it is said controller may request additional info, and now that it is not obliged to do so?}
%\item Answering to a SAR. Whenever a data subject provides additional data that enables their identification, the controller shall not refuse their SAR (Article 11.2 of GDPR). \kao{unclear: only valid if the user has to provide additional info? what if they were already identifiable from the start?}
%\end{enumerate}











==> zhang.tex <==

\subsection{Confusion}



\noindent
\textbf{Assumption 1.}
It is  common to assume that a full name is enough to identify an individual (see~\cite{WP29}) and therefore, an individual full name is often the textbook example  illustrating the definition of personal data. This assumption is often true in Europe and in western countries: even if it is not impossible, it is rare to find two persons sharing the same first and last name. 

\noindent
\textbf{Naming tradition and demography in China.}
The situation is different in other countries and particularly in China. %Common 
People in China are known by the term \emph{``hundred common name''} which refers to the fact that the 100 most popular last names are used by 85.9\% of the population (in 2019\footnote{\url{http://gat.ah.gov.cn/public/7081/40201012.html} last acceded April 2021}).  In China, it is very probable to find somebody which shares the first and last name -- there are many individuals  who share the same full name Zhang Wei for instance. Table~\ref{tab:zhang} shows the most popular full names in China in 2007\footnote{\url{http://news.cctv.com/society/20070725/105888.shtml} last acceded April 2021} and in 2019\footnote{\url{http://gat.ah.gov.cn/public/7081/40201012.html} last acceded April 2021}. 

\begin{table}[ht]
    \centering
    \begin{tabular}{r|r|r}
    \textbf{Surnames}     & \textbf{\#individuals (2007)} & \textbf{\#individuals (2019)}\\ \hline
    Zhang Wei       &   290.607 &   294.282     \\  
    Wang Wei        &   281.568 &   287.101  \\
    Wang Fang       &   268.268 &   271.550 \\
    Li Wei          &   260.980 &   266.037\\
    \end{tabular}
    \caption{Most popular full names in China (2007 and 2019).}
    \label{tab:zhang}
\end{table}

A full name is not enough to identify somebody uniquely in China. 
If the first and last name collisions exist, one might think that it is enough to simply add extra information, suck like the birth date to uniquely identify an individual in China, %though it is  not enough to distinguish. 
Data controllers would simply ask the birth date to the subjects, alongside their full names, to remove any ambiguity about the subjects identity, though the birth data is not distinguishable. %Unfortunately, demography in China 
Between 2007 and 2019, 5533 individuals with the name Wang Wei were born in China. This statistic does not take into account the number of Wang Wei who died during this period of time and we were unable to find such a statistic. Assuming that the births are equally distributed over the years, it gives us  461 births per year on average. Due to the Pigeonhole principle, we have necessarily people named Wang Wei having the same birth date. The scale of this effect might be even higher if we consider a more accurate model for the distribution of the birth dates~\cite{Flajolet1992,Holst1995}. Still, our simple computation is enough to highlight the problem. 

%How does naming tradition and demography affect the GDPR and subject access right? 
\noindent
\textbf{Denial of access.} The scope of the GDPR creates opportunity for impersonation attacks and consequent denial of access. It creates an army of ``clones'' of people having almost the same official identification document, wherein the data of an individual can be claimed by other individuals which share the same full name and the same birth date.
Let's consider that a data controller located in Europe is collecting and processing the data of a honest Zhang Wei (Figure~\ref{fig:clone}). It is possible for another subject named Zhang Wei$^{\star}$ to submit a request to obtain the data from the honest Zhang Wei. If both identification documents are very similar, the data controller will send the data from the honest Zhang Wei to the malicious one. 

\begin{figure}[ht]
\centering
\input{fig/clone.pdf_t}
\caption{Impersonation attack by a sharing the same full name. A subject named Zhang Wei use a service but it is another one named Zhang Wei who request the data and obtained them from the data controller.}\label{fig:clone}
\end{figure}



A data controller who uses document-based authentication created by a trusted third party may systematically deny a SAR from subjects with an Asian name. It might consider that the official document does not help to identify uniquely the subject making the request. 

